On Complexity of 1-Center in Various Metrics

We consider the classic 1-center problem: Given a set $P$ of $n$ points in a metric space find the point in $P$ that minimizes the maximum distance to the other points of $P$. We study the complexity of this problem in $d$-dimensional $\ell_p$-metrics and in edit and Ulam metrics over strings of length $d$. Our results for the 1-center problem may be classified based on $d$ as follows. $\bullet$ Small $d$: Assuming the hitting set conjecture (HSC), we show that when $d=\omega(\log n)$, no subquadratic algorithm can solve 1-center problem in any of the $\ell_p$-metrics, or in edit or Ulam metrics. $\bullet$ Large $d$: When $d=\Omega(n)$, we extend our conditional lower bound to rule out subquartic algorithms for 1-center problem in edit metric (assuming Quantified SETH). On the other hand, we give a $(1+\epsilon)$-approximation for 1-center in Ulam metric with running time $\tilde{O_{\varepsilon}}(nd+n^2\sqrt{d})$. We also strengthen some of the above lower bounds by allowing approximations or by reducing the dimension $d$, but only against a weaker class of algorithms which list all requisite solutions. Moreover, we extend one of our hardness results to rule out subquartic algorithms for the well-studied 1-median problem in the edit metric, where given a set of $n$ strings each of length $n$, the goal is to find a string in the set that minimizes the sum of the edit distances to the rest of the strings in the set.

==> l_1-constant.tex <==
\section{1-Center for $\ell_1$ Metric in Low Dimension}\label{sec:lowdim}
In this section, we give an algorithm that runs in time $O(2^dnd)$ and solves 1-center exactly in $\ell_1$-metric when the dimension is $d$ and the number of points is $n$. Our algorithm is based on a very simple observation: Let $v^0, v^1, \ldots, v^{2^d-1}$ be $2^d$ vectors of size $d$ such that each vector $v^i$ is the bit representation of value $i$ in base $2$. We define $2^d$ functions $f_0, f_1, f_2, \ldots, f_{2^d-1}$ such that the input to every function $f_i$ is a $d$-dimensional point $u$ and its output is determined in the following way:
\[f_i(u)  = \sum_{1 \leq j \leq d, v^i_j = 1} u_j - \sum_{1 \leq j \leq d, v^i_j = 0} u_j.\]

It follows from the definition that for any two points $x$ and $y$ the following conditions hold:
\begin{itemize}
	\item $\forall 0 \leq i < 2^d, \ell_1(x,y) \geq f_i(x) - f_i(y)$.
	\item $\exists 0 \leq i < 2^d$ such that $\ell_1(x,y) = f_i(x) - f_i(y)$.
\end{itemize}
where $\ell_1(x,y)$ is the distance of points $x$ and $y$ under $\ell_1$ metric. Let $p_1, p_2, \ldots, p_n$ be the input points. It follows that for each point $x$ on the plane, the point $p_j$ that maximizes its distance from $x$ has the highest value for at least one $f_i$. Based on this fact, our algorithm is as follows: we iterate over all $n$ points and for each function $f_i$ we find the point that maximizes the value of $f_i$. Next, for each of the $n$ points we find the farthest point to it by computing its distance to $2^d$ points that are the extreme points for the functions. Our algorithm takes time $O(2^dnd)$.

%\thml*

\begin{proof}[Proof of Theorem~\ref{thm:l1center}]
The runtime of the algorithm is trivially bounded by $O(2^dnd)$. Here we give a formal proof for the properties that we mentioned earlier. We first show that for each pair of points $x$ and $y$, and any $0 \leq i < 2^d$, the $\ell_1$ distance of $x$ and $y$ is lower bounded by $f_i(x) - f_i(y)$. This follows from the following inequalities:

\begin{equation*}
\begin{split}
f_i(x) - f_i(y)  & =  \sum_{1 \leq j \leq d, v^i_j = 1} x_j - \sum_{1 \leq j \leq d, v^i_j = 0} x_j  - \sum_{1 \leq j \leq d, v^i_j = 1} y_j + \sum_{1 \leq j \leq d, v^i_j = 0} y_j \\
					   & =  \sum_{1 \leq j \leq d, v^i_j = 1} (x_j - y_j) + \sum_{1 \leq j \leq d, v^i_j = 0} (y_j - x_j) \\
					   & \leq \sum_{1 \leq j \leq d} |x_j - y_j|\\
					   & = \ell_1(x,y).
\end{split}
\end{equation*}

To prove the second property, let for a point $x$ and a point $y$, $v$ be a 0/1 bit vector such that $v_j = 1$ if $x_j \geq y_j$ and $v_j = 0$ otherwise. Let the base-10 value of vector $v$ be $i$ and thus $v^i= v$. We then show that $\ell_1(x,y) = f_i(x) - f_i(y)$ as follows: 

\begin{equation*}
\begin{split}
f_i(x) - f_i(y)  & = \sum_{1 \leq j \leq d, v^i_j = 1} x_j - \sum_{1 \leq j \leq d, v^i_j = 0} x_j  - \sum_{1 \leq j \leq d, v^i_j = 1} y_j + \sum_{1 \leq j \leq d, v^i_j = 0} y_j \\
& =  \sum_{1 \leq j \leq d, v^i_j = 1} (x_j - y_j) + \sum_{1 \leq j \leq d, v^i_j = 0} (y_j - x_j) \\
& = \sum_{1 \leq j \leq d} |x_j - y_j|\\
& = \ell_1(x,y).
\end{split}
\end{equation*}

To show that for each point $x$, the farthest point from $x$ is the extreme point for one function $f_i$ we bring the following argument: Let $p_j$ be the point that is the farthest from $x$ and $f_i$ be the function such that $f_i(p_j) - f_i(x) = \ell_1(p_j,x)$. Now, consider a point $p_{j'}$ that maximizes the value of $f_i$. Thus, we have:

\begin{equation*}
\begin{split}
f_i(p_{j'}) - f_i(x)  & \geq f_i(p_{j}) - f_i(x)\\
& = \ell_1(p_{j},x).
\end{split}
\end{equation*}
which implies that the distance of $p_{j'}$ and $x$ is at least as large as the distance of $p_j$ and $x$ by $\ell_1(p_{j'},x) \geq |f_i(p_{j'}) - f_i(x)|$.
\end{proof}

As a corollary of Theorem~\ref{thm:l1center}, one can find the farthest pair of the points with the same algorithm.

\corl*
\begin{proof}[Proof of Corollary~\ref{thm:l1diameter}]
	The algorithm is  the same as the algorithm of Theorem~\ref{thm:l1center} except that instead of finding a point that minimizes the distance to the farthest point, we find the point that maximizes the distance to the farthest point. The proof is exactly the same. 
\end{proof}


